Output beam shaping of a multimode fiber amplifier

Multimode fibers provide a promising platform for realizing high-power laser amplifiers with suppressed nonlinearities and instabilities. The potential degradation of optical beam quality has been a major concern for highly multimode fiber amplifiers. We show numerically that the beam propagation factor M2 of a single-frequency multimode fiber amplifier can be reduced to nearly unity by shaping the input or output beam profile with spatial phase-masks. Our method works for narrowband multimode fiber amplifiers with strong gain saturation, pump depletion, random mode coupling and polarization mixing. The numerical results validate our approach of utilizing highly multimode excitation to mitigate nonlinear effects in high-power fiber amplifiers and performing input wavefront shaping to control output beam profile and polarization state.

==> setup.tex <==
% MATH
\newcommand{\expect}[2][]{\ensuremath{\mathbb{E}_{#1}\left[#2\right]}}
\newcommand{\inv}[1]{\ensuremath{#1^{-1}}}
\newcommand{\herm}[1]{\ensuremath{#1^{\mathsf{H}}}}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\positive}[1]{\ensuremath{\left[#1\right]^{+}}}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\mutI}{\mathbb{I}}
\DeclareMathOperator{\svd}{svd}

\newcommand{\reals}{\ensuremath{\mathds{R}}}
\newcommand{\complexes}{\ensuremath{\mathds{C}}}
\newcommand{\e}{\ensuremath{\mathrm{e}}}

\newcommand{\M}{\ensuremath{\bm{\tilde{M}}}}
\newcommand{\X}{\ensuremath{\bm{X}}}
\newcommand{\Y}{\ensuremath{\bm{Y}}}
\newcommand{\Z}{\ensuremath{\bm{Z}}}

\newcommand*{\tm}{\ensuremath{\mathrm{TM}}}

\renewcommand{\vec}{\mathbf}
\renewcommand{\Re}{\mathrm{Re}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COLORS
\definecolor{plot0}{HTML}{1bb34c}
\definecolor{plot1}{HTML}{242bb3}
\definecolor{plot2}{HTML}{b3120e}
\definecolor{plot3}{HTML}{cc9f2b}
\definecolor{plot4}{HTML}{27AFB3}
% \definecolor{plot0}{HTML}{339933}
% \definecolor{plot1}{HTML}{004488}
% \definecolor{plot2}{HTML}{DDAA33}
% \definecolor{plot3}{HTML}{BB5566}
% \definecolor{plot4}{HTML}{8888AA}
\definecolor{plot0}{HTML}{004488}
\definecolor{plot1}{HTML}{DDAA33}
\definecolor{plot2}{HTML}{BB5566}
\definecolor{plot3}{HTML}{000000}
\definecolor{plot4}{HTML}{AAAAAA}

\pgfplotscreateplotcyclelist{lineplot cycle}{%
{plot0, thick, mark=*},%, mark size=1.5pt},
{plot1, thick, mark=square*},%, mark size=1.3pt},
{plot2, thick, mark=triangle*, mark size=2.3pt},
{plot3, thick, mark=diamond*},%, mark size=1.5pt},
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TIKZ
\usetikzlibrary{shapes, arrows, positioning, calc, external}
\tikzset{%
	block/.style    = {draw, rectangle, minimum height=3em, minimum width=3em},
	sum/.style      = {draw, thick, circle, inner sep=.1em},
}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{fillbetween}

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 


\newcommand{\todo}[2][]{
	\if\relax\detokenize{#1}\relax
	{\color{red}[TODO: #2]}%
	\else
	{\color{red}[TODO (#1): #2]}%
	\fi
}
\newcommand{\note}[1]{{\color{orange}#1}}

\definecolor{change}{HTML}{0096b8}
\newcommand{\change}[1]{\ignorespaces{\color{change}#1}}
